Implicit Generation and Generalization in Energy-Based Models

Energy based models (EBMs) are appealing due to their generality and simplicity in likelihood modeling, but have been traditionally difficult to train. We present techniques to scale MCMC based EBM training on continuous neural networks, and we show its success on the high-dimensional data domains of ImageNet32x32, ImageNet128x128, CIFAR-10, and robotic hand trajectories, achieving better samples than other likelihood models and nearing the performance of contemporary GAN approaches, while covering all modes of the data. We highlight some unique capabilities of implicit generation such as compositionality and corrupt image reconstruction and inpainting. Finally, we show that EBMs are useful models across a wide variety of tasks, achieving state-of-the-art out-of-distribution classification, adversarially robust classification, state-of-the-art continual online class learning, and coherent long term predicted trajectory rollouts.

==> figText/cifar10_class.tex <==
\begin{table}
%\setlength{\tabcolsep}{6pt}
\centering
\begin{tabular}{lcccc}
    \toprule
    \# & Baseline & FT & Baseline + DA & FT + DA\\
    \midrule
    Accuracy & 83.6 & 86.5 & 89.7 & 90.2 \\
    \bottomrule
\end{tabular}
\caption{\small Test Accuracy on CIFAR10 with or without finetuning (FT) with or without data augmentation (DA). We using horizontal flip and random crop data augmentations. Energy based fine-tuning allow better generalization.}
\label{tbl:cifar10_class}
\end{table}


==> figText/completions.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1.0\linewidth]{fig/completions.pdf}
\caption{\small Illustration of image completions on conditional ImageNet model. Our models exhibit diversity in inpainting.} 
\label{fig:completions}
\end{center}
\end{figure}

==> figText/compositional.tex <==
\begin{figure}%{0.5\textwidth}
\begin{center}
\includegraphics[width=0.8\linewidth]{fig/compositional.pdf}
\caption{\small GT = Ground Truth. Images of cross product generalization of size-position (left panel) and shape-position (right panel).}
\label{fig:comb_im}
\end{center}
\vspace{-10pt}
\end{figure}

==> figText/cross_class.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.6\linewidth]{fig/cross_class.pdf}
\caption{\small Illustration of cross-class implicit sampling on a conditional EBM. The EBM is conditioned on a particular class but is initialized with an image from a separate class.} 
\label{fig:cross_class}
\end{center}
\end{figure}

==> figText/decker.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=0.8\linewidth]{fig/decker.pdf}
\caption{\small Illustration of images from each of the out of distribution dataset.} 
\label{fig:decker}
\end{center}
\end{figure}

==> figText/decorrupt.tex <==
\begin{figure}[h]
\includegraphics[width=1.0\linewidth]{fig/decorrupt.pdf}
\caption{\small EBM image restoration on images in the \textbf{test} set via MCMC. The right column shows failure (approx. 10\% objects change with ground truth initialization and 30\% of objects change in salt/pepper corruption or in-painting. Right column shows worst case of change.)} 
\label{fig:decorrupt}
\vspace{-5mm}
\end{figure}


==> figText/hand_uncond_cond.tex <==
\begin{figure}
\begin{center}
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{fig/cond_frechet.pdf}
\end{subfigure}%
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{fig/uncond_frechet.pdf}
\end{subfigure}
\caption{\small Conditional and Unconditional Modeling of Hand Manipulation through Frechet Distance}
\label{fig:cond_uncond_hand}
\end{center}
\vspace{-5pt}
\end{figure}

==> figText/image_samples.tex <==
\begin{figure}[h]
\begin{center}
\begin{subfigure}{0.23\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{fig/glow_uncond.png}
    \caption{GLOW \citep{kingma2018glow} samples}
\end{subfigure}%
\begin{subfigure}{0.23\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{fig/uncond_sample.png}
    \caption{EBM samples}
\end{subfigure}
\begin{subfigure}{0.23\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{fig/uncond_sample_ensemble.png}
    \centering
    \caption{Last 10 snapshots EBM samples}
    \label{fig:hist}
\end{subfigure}
\begin{subfigure}{0.23\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{fig/replay_buffer.png}
    \centering
    \caption{Samples for replay buffer during unconditional training}
    \label{fig:replay}
\end{subfigure}
% \includegraphics[width=0.8\linewidth]{fig/uncond_gen.pdf}
% \caption{Illustration of generation of images by unconditional model.} 
\caption{\small Illustrations of image generation from GLOW as compared to our EBM models for unconditional generation on CIFAR-10. Our models are able to more accurately generate objects.}
\label{fig:qual_images}
\end{center}
\end{figure}

==> figText/joint.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1.0\linewidth]{fig/joint.pdf}
\caption{\small Samples from joint distribution of 4 independent conditional EBMs on scale, position, rotation and shape (left) with associated ground truth rendering (right).} 
\label{fig:joint}
\end{center}
\end{figure}


==> figText/joint_traj_class.tex <==
\begin{figure}
\begin{center}
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=0.8\linewidth]{fig/traj.pdf}
\caption{Multistep time series prediction MSE errors (\textbf{log} scale). EBMs show out of distribution generalization by reduced long term rollout error.} 
\label{fig:traj_plots}
\end{subfigure} 
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=1.0\linewidth]{fig/cross_class.pdf}
\caption{\small Illustration of cross class mapping using GEO on a conditional EBM. The EBM is conditioned on a particular class but is initialized with an image from a separate class(left). Additional images in \fig{fig:cross_class_more}} 
\label{fig:cross_class}
\end{subfigure}
\end{center}
\end{figure}


==> figText/kl_effect.tex <==
\begin{figure}
\minipage{0.5\linewidth}
  \includegraphics[width=\linewidth]{fig/energy_hist/test_50_nokl.png}
\endminipage\hfill
\minipage{0.5\linewidth}
  \includegraphics[width=\linewidth]{fig/energy_hist/test_50_kl.png}
\endminipage
\caption{\small Energy distributions after training without (\textbf{left}) and with (\textbf{right}) KL objective in (\ref{eq:kl}) over \emph{dSprites} dataset.} 
\label{fig:kl_effect}
\vspace{-8pt}
\end{figure}

==> figText/online_tbl.tex <==
\begin{table}
%\setlength{\tabcolsep}{6pt}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
    \toprule
    \# & EWC & SI & NAS & LwF & VAE & EBM (ours) \\
    \midrule
    Accuracy & 19.80 (0.05) & 19.67 (0.09) &  19.52 (0.29) & 24.17 (0.33) &  40.04 (1.31) & 64.99 (4.27) \\
    
    \bottomrule
\end{tabular}
}
\caption{\small Comparison of various continual learning benchmarks with conditional EBM/VAE training  with EWC \citep{kirkpatrick2017overcoming}, SI \citep{}, NAS \citep{schwarz2018progress} and LwF \citep{li2018learning}. Values averaged acrossed 10 seeds reported as mean (standard deviation).}
\label{tbl:online_tbl}
\end{table}


==> figText/teaser.tex <==
\begin{figure}[H]
\begin{center}
    \includegraphics[width=0.7\linewidth]{fig/teaser.pdf}
\end{center}

\caption{\small Images of Langevin Dynamic Sampling (gradient based) on a class condition EBMs initialized with random image and image of different class.}  
\vspace{-10pt}
\label{fig:teaser}
\end{figure}


==> figText/traj_plots.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\begin{center}
\includegraphics[width=1.0\linewidth]{fig/traj.pdf}
\caption{\small Multistep time series prediction MSE errors (\textbf{log} scale). EBMs show out of distribution generalization by reduced long term rollout error.} 
\label{fig:traj_plots}
\end{center}
\end{wrapfigure}
% \vspace{-7mm}

==> text/notes.tex <==
Contributions:

Learning how to generate samples through optimization
EBM for representation learning

Iterative refined for world models


CogSci story:

- Brain does internal predictions of the future
- it's so good at it because 1) it has well-designed priors (i.e. lighting, geometry, etc) and 2) because it has well-designed processes for doing it (i.e. iteratively refine with feedback and build up generated sample over time)
- we are investigating the #2
- tools of optimization and EMBs provide a path to do this
- our contribution: is the application of these ideas to physical system prediction or generation, and image generation
- we are learning in a contrastive manner inspired by wake-sleep learning and could provide explanation for theories of sleep
- we find that our EBMs learn useful internal representations that can be fine-tuned to tasks (we use image classification task, but it can be useful for abstract control/planning)
- [it can be thought of as learning core intuitive concepts/knowledge about the world?]
- 
- [interpretation as implicit integrator, or as a deconv?]

Contributions:
- explore implicit stochastic sampling for agent's prediction/generation processes

Experiments:
- domains:
    - MNIST
    - Omniglot
    - CIFAR10
    - point mass 1
    - point mass 8?
    - dsprites?
    - fetch
    - shadowhand?
    
- 


Experiments to Run:
Images
    - CIFAR10 finetuning - quantative
    - qualitative CIFAR10 Images
    - CIFAR10 image generation scores - FID/Inception (Likelihood?)
    - CIFAR10 class conditional images - FID/Inception
    - Qualitative visualization of image traversal on labels
    - Evaluation of classification 
    - Decorruption: add salt and pepper noise (10 percent) and hole inpainting
Trajectories
    - point mass 1 / 8 MSE / comparison over other methods
    - comparison of differnt different optimization methods: SGD, MPPI
    - Plot: rollout MSE feedforward vs energy autoregressive vs energy autoregressive + finetuning for 100 trials with error bars Expected result: energy does diverge, but some samples are still good, whereas feedforward diverges consistently
    - Finetuning energy function to regress particle parameters

\begin{enumerate}
    \item 
\end{enumerate}
